Entropy-Preserving and Entropy-Stable Relaxation IMEX and Multirate Time-Stepping Methods

We propose entropy-preserving and entropy-stable partitioned Runge--Kutta (RK) methods. In particular, we extend the explicit relaxation Runge--Kutta methods to IMEX--RK methods and a class of explicit second-order multirate methods for stiff problems arising from scale-separable or grid-induced stiffness in a system. The proposed approaches not only mitigate system stiffness but also fully support entropy-preserving and entropy-stability properties at a discrete level. The key idea of the relaxation approach is to adjust the step completion with a relaxation parameter so that the time-adjusted solution satisfies the entropy condition at a discrete level. The relaxation parameter is computed by solving a scalar nonlinear equation at each timestep in general; however, as for a quadratic entropy function, we theoretically derive the explicit form of the relaxation parameter and numerically confirm that the relaxation parameter works the Burgers equation. Several numerical results for ordinary differential equations and the Burgers equation are presented to demonstrate the entropy-conserving/stable behavior of these methods. We also compare the relaxation approach and the incremental direction technique for the Burgers equation with and without a limiter in the presence of shocks.

==> makefile <==
BASENAME = main
REPORT = main_report

do:: all

report::
	pdflatex ${REPORT}

pdf::
	pdflatex ${BASENAME}

all::
	pdflatex ${BASENAME}
	bibtex ${BASENAME}
	pdflatex ${BASENAME}
	pdflatex ${BASENAME}

response::
	pdflatex response
	bibtex   response
	pdflatex response
	pdflatex response

arxiv::
	tar -czf arxiv.tar.gz *

#DIFFDIR=./0-original-08-19-2021
DIFFDIR=./1-revision1-03-14-2022/revision-10June2022

# Add the following preamble to diff files 
#\providecommand{\DIFaddEQ}[1]{{\protect\color{blue}\uline{#1}}} %DIF PREAMBLE
#\providecommand{\DIFdelEQ}[1]{{\protect\color{red}\uline{#1}}}
# or change uwave to uline
# \providecommand{\DIFaddtex}[1]{{\protect\color{blue}\uline{#1}}} %DIF PREAMBLE
diff:
	latexdiff ${DIFFDIR}/main.tex main.tex > ./diff_main.tex
	#latexdiff --math-markup=0  ${DIFFDIR}/main.tex main.tex > ./diff_main2.tex


clean::
	rm -f ${BASENAME}.sync*
	rm -f ${BASENAME}.fdb*
	rm -f ${BASENAME}.fls
	rm -f ${BASENAME}.bbl
	rm -f ${BASENAME}.blg
	rm -f ${BASENAME}.log
	rm -f ${BASENAME}.pdf
	rm -f ${BASENAME}.aux
	rm -f ${BASENAME}.out
	rm -f ${BASENAME}.tex~
	rm -f ${BASENAME}.spl


